Social Media, Content Moderation, and Technology

This paper develops a theoretical model to study the economic incentives for a social media platform to moderate user-generated content. We show that a self-interested platform can use content moderation as an effective marketing tool to expand its installed user base, to increase the utility of its users, and to achieve its positioning as a moderate or extreme content platform. The optimal content moderation strategy differs for platforms with different revenue models, advertising or subscription. We also show that a platform's content moderation strategy depends on its technical sophistication. Because of imperfect technology, a platform may optimally throw away the moderate content more than the extreme content. Therefore, one cannot judge how extreme a platform is by just looking at its content moderation strategy. Furthermore, we show that a platform under advertising does not necessarily benefit from a better technology for content moderation, but one under subscription does. This means that platforms under different revenue models can have different incentives to improve their content moderation technology. Finally, we draw managerial and policy implications from our insights.

==> ext_boycott.tex <==
%\section{Extensions} \label{sec: exten}

\section{Advertisers' Preference for Content Moderation}\label{sec: ad value and extr}


In the main model, we assumed that every user had the same advertising value to advertisers. However, the recent boycott of advertisers on Facebook against the wide spread of hate content may indicate that extreme users who post a lot of extreme content may not be as valuable as moderate users to advertisers. In order to consider the possibility that advertisers have a preference on moderate users over extreme users, we assume in this extension that the advertising value of users is decreasing in the average extremity level of the user community, i.e., the advertising value per user becomes

$$\tilde{a}(\overline{x})=a'-\beta\overline{x}=a'-\beta\frac{x^A+y}{2},$$
where $\beta>0$.

Therefore, if the platform chooses the advertising-based model, its revenue now becomes
\begin{equation}
    \tilde{\pi}^A(y)=\tilde{a}(\overline{x})X^A(y)=\Big[a'-\beta\frac{x^A(y)+y}{2}\Big](y-x^A(y))
\end{equation}

By construction, this makes the advertising-based business model less favorable compared to the subscription-based one. However, will this boycott from advertisers necessarily induce a stricter content moderation policy of the platform? We answer the question in Proposition \ref{prop:boycott}.

\begin{proposition}\label{prop:boycott}
{\bf \em (Advertisers' Preference for Content Moderation)} Suppose the advertising value per user is decreasing in $\overline{x}$, the optimal content moderation behavior ($\tilde{y}^{A*}$) of an advertising-supported platform is described as follows:
\begin{itemize}
    \item When $\alpha\leq\sqrt{2v}$,
    \begin{equation}
   \tilde{y}^{A*} = 
    \begin{cases}
    \sqrt{2v} & \text{if $\beta\leq a'\sqrt{\frac{1}{2v}}$;} \\
    \frac{a'}{\beta}(<\sqrt{2v}) & \text{if $\beta>a'\sqrt{\frac{1}{2v}}$.} 
  \end{cases}
\end{equation}
\item When $\alpha>\sqrt{2v}$,
    \begin{equation}
   \tilde{y}^{A*} = 
    \begin{cases}
    1 & \text{if $\beta\leq a'\frac{\sqrt{1+\alpha^2-2v}-1}{\alpha}$;} \\
     a'\sqrt{\frac{\alpha^2-2v}{\alpha\beta(2a'+\alpha\beta)}}(<1) & \text{if $a'\frac{\sqrt{1+\alpha^2-2v}-1}{\alpha}<\beta\leq a'(\sqrt{\frac{1}{2v}}-\frac{1}{\alpha})$;} \\
      \sqrt{2v}(<a'\sqrt{\frac{\alpha^2-2v}{\alpha\beta(2a'+\alpha\beta)}}) & \text{if $a'(\sqrt{\frac{1}{2v}}-\frac{1}{\alpha})<\beta\leq a'\sqrt{\frac{1}{2v}}$;} \\
    \frac{a'}{\beta}(< \sqrt{2v}) & \text{if $\beta>a'\sqrt{\frac{1}{2v}}$.} 
  \end{cases}
\end{equation}
\end{itemize}
\end{proposition}

Comparing Proposition \ref{prop:boycott} to Proposition \ref{prop:ad_eq}, we first find that the boycott has to be severe enough ($\beta$ large enough) in order to induce a more strict content moderation policy; otherwise, the boycott does not affect the moderation behavior of the platform at all. Also, we can see that the boycott has the potential to make a platform which did not do content moderation before do moderate the content, as long as $\beta$ is large enough.

We carry out the following analysis to see why we need a high enough $\beta$ to change the content moderation policy of the platform. We take the case when $\alpha\leq \sqrt{2v}$ as an example, since the other case ($\alpha>\sqrt{2v}$) is in the same spirit. Starting from the optimal moderation level ($y^{A*}$) when the advertising value is independent of content extremity, the platform for sure will not make the moderation policy more lenient since by doing so it cannot increase its market size and also decreases the advertising value per user. To decide whether it is more profitable to perform more content moderation, i.e., a more strict moderation policy, one can compare the marginal gain and the marginal loss when setting a slightly more strict moderation policy $y=y^{A*}-\Delta y$. The marginal loss is $\Delta y(a'-\beta\frac{X^{A*}}{2})$, which comes from the fact that some users will leave the platform. The marginal gain is $(X^{A*}-\Delta y)\beta\frac{\Delta y}{2}$, which comes from the increased advertising value of the remained users (recall that $X^{A*}$ is the size of the platform's user base in the benchmark case). A more strict moderation policy is only more profitable when $(X^{A*}-\Delta y)\beta\frac{\Delta y}{2}>\Delta y(a'-\beta\frac{X^{A*}}{2})$, which is equivalent to $\beta>\frac{a'}{X^{A*}}$ when $\Delta y$ is small. Clearly, $\frac{a'}{X^{A*}}$ decreases in $X^{A*}$, which implies that the boycott from advertisers is more likely to be effective when the platform has a larger user base. 





==> ext_mixed_model.tex <==
\subsection{Advertising and Subscription Revenue Sources Together}\label{sec:mixed}

A number of social media platforms operate by revenues from both advertising and subscription fees.  YouTube, for instance, earns revenue from both sources, offering a basic ad-supported version and a premium version where users have more control (YouTube Premium).\footnote{\url{https://www.youtube.com/premium}} There has also been discussions about Facebook introducing an ad-free paid version of its product in recent years.\footnote{\url{https://www.washingtonpost.com/news/the-fix/wp/2018/04/14/would-you-pay-18-75-for-ad-free-facebook/},\url{https://www.vox.com/2019/2/20/18233640/mark-zuckerberg-explains-ad-free-facebook}} LinkedIn, a professional networking platform, again earns both revenues from subscription and advertising. So it is worthwhile to examine how a hybrid revenue model would alter our findings. 


We assume that in a hybrid model, users self select to either participate on the platform without paying in exchange for seeing ads, or see no ads but pay a subscription fee. 
Suppose now that when seeing ads, a user's utility from participating in the social media platform is discounted by a factor $\delta\in[0,1]$. That is, a user at $x$'s utility becomes $(1-\delta)U(x)$ if she chooses to use the free version, where $U(x)$ is given in equation \eqref{eq:utility_fcn}. Therefore, $\delta$ indicates how ``advertisement-averse'' the users are when they are using the platform -- a larger $\delta$ means users feel more negative about ads. On the other hand, if user $x$ chooses to pay for an ad-free version of the platform, her net utility is $U(x)-p$, where $p$ is the subscription fee. A user self selects to participate in the platform if and only if her net utility is positive.

If the platform chooses a hybrid model, it sets both the content moderation policy $y$ and the subscription fee $p$. We assume, similar to the benchmark model, the moderation algorithm is perfect in detection.

Similar to Lemma \ref{lem:config}, we can show that the total user base, including both the users who pay and those do not pay, is a continuum between $x^H(y)$ and $y$, where $x^H(y)$ solves $(1-\delta) U(x^H(y))=0$. Among all the users, since $U(x)$ is increasing in $x$, users who pay for the ad-free version are those with large $x$. The utility function in a fulfilled expectations equilibrium as specified in equation (\ref{eq:utility_fcn_eqm}) still applies.
Therefore, the configuration of user base is as shown in Figure \ref{fig:config_hybrid}: users between $x^H(y)$ and $\hat{x}(y,p)$ (in light gray) use the free version with ads and users between $\hat{x}(y,p)$ and $y$ (in dark gray) pay for the ad-free version, where $\hat{x}(y,p)$ solves
\begin{equation}
    (1-\delta)U(\hat{x})=U(\hat{x})-p.
\end{equation}
The platform's profit-maximization problem when it chooses a hybrid business model is thus
\begin{equation}
    \max_{y,p}\pi^H=a\Big(\hat{x}(y,p)-x^H(y)\Big)+p\Big(y-\hat{x}(y,p)\Big).
\end{equation}
%where denote the optimal profit in a hybrid model as $\pi^{H*}$.

\begin{figure}[h]
\caption{Illustration of the platform's user base (hybrid model)}
    \label{fig:config_hybrid}
    \centering
\begin{tikzpicture}[scale=0.75]

\path [fill=lightgray] (4,0) -- (2,0) -- (2,1.5) -- (4,1.5);
\path [fill=gray] (7,0) -- (4,0) -- (4,1.5) -- (7,1.5);

\draw (0,0) node [below] {$0$} -- (8,0) node [below] {$1$} -- (8,1.5) -- (0,1.5)  --cycle;
\draw (4,0) node [below] {$\hat{x}(y,p)$} -- (4,1.5);
\draw (2,0) node [below] {$x^H(y)$} -- (2,1.5);
\draw (7,0) node [below] {$y$} -- (7,1.5);


\end{tikzpicture}
    
\end{figure}



The following proposition describes the optimal content moderation policy of the platform which implements a hybrid business model.

\begin{proposition}\label{prop:hybrid_y} {\bf \em (Content Moderation under a Hybrid Revenue Model)} Let $\hat{a}$ be a constant.
For a platform with advertising and subscription revenues,

\begin{itemize} 
\item if user heterogeneity is low ($\alpha\leq\overline{\alpha}$)  or if it is intermediate ($\overline{\alpha}<\alpha\leq\sqrt{2v}$) and ad-revenue per customer is high ($a>\hat{a}$), content moderation is identical to that in an ad-only revenue model ($y^{H*}=\sqrt{2v}$)

\item If user heterogeneity is high ($\alpha>\sqrt{2v}$) or it is intermediate ($\overline{\alpha}<\alpha\leq\sqrt{2v}$) but ad-revenue per user is low ($a<\hat{a}$), then there is no content moderation ($y^{H*}=1$). 
\end{itemize}
\end{proposition}

Proposition \ref{prop:hybrid_y} shows that content moderation policy for a hybrid-revenue platform is similar to that for an advertising-supported platform when $\alpha$, the heterogeneity in posting utility among users, is either small or intermediate with sufficient ad-revenues. When $\alpha$ is intermediate, we know from Corollary \ref{cor:ad vs subs} that the advertising and subscription-supported platforms diverge in content moderation policy. For a hybrid model, it follows the subscription model (anti content moderation) when $a$, the advertising value per user, is low, while follows the advertising model (pro content moderation) when $a$ is high. Intuitively, this is because a hybrid model is a mixture of the two basic models, and behaves more like the advertising (subscription) model when users' advertising value is high (low).

Suppose that the platform has the opportunity to choose its business model before setting its content moderation policy, and the hybrid model is another alternative in addition to advertising and subscription models, comparing $\pi^{A*}$, $\pi^{S*}$, and $\pi^{H*}$. Note that when the subscription fee is set very high, the hybrid model simply reduces to the advertising-supported model. To avoid such dominance of the hybrid model over the advertising-only model, we assume that if, in the equilibrium of a hybrid business model no user pays for the ad-free version, the platform will simply choose the advertising-only model for the ease of operation. 

An examination of profits ($\pi^{A*}$, $\pi^{S*}$, and $\pi^{H*}$) and their relationship with the advertising value $a$ confirms the following intuition: the advertising model is preferred when $a$ is high, the subscription model is preferred when $a$ is low. The hybrid model can dominate the other alternatives iff $a$ is intermediate. There are two possibilities, as shown in Figure \ref{fig:mixed_choice_1}: in Scenario 1, the hybrid model is indeed preferred for intermediate $a$, but in Scenario 2, the hybrid model is never preferred for whatever $a$.

\begin{figure}[h]
\caption{Two possible scenarios in business model choice}\label{fig:mixed_choice_1}
\centering
\includegraphics[width=\textwidth]{figures/mixed_choice_1.PNG}
\end{figure}


When will each scenario happen? Or, when does the hybrid model have the opportunity to be chosen by the platform? The following proposition answers these questions. 

\begin{proposition}\label{prop:hybrid_model_choice}
{\bf \em (Revenue model choice with the hybrid model) } There exists $\overline{\delta}>0$, such that 
\begin{itemize}
    \item if $\delta\leq\overline{\delta}$, the platform chooses the subscription model when $a\leq a_1$, and the advertising model when $a>a_1$, where $a_1$ is independent of $\delta$;
    \item if $\delta>\overline{\delta}$, the platform chooses the subscription model when $a\leq a_2$, the hybrid model when $a_2<a\leq a_3$, and the advertising model when $a>a_3$, where $a_2$ is decreasing in $\delta$ and $a_3$ is increasing in $\delta$.
\end{itemize}
\end{proposition}

From Proposition \ref{prop:hybrid_model_choice}, we see first that the hybrid model can be preferred when the advertising value per user is intermediate. However, this does not always happen. There is only room for the hybrid model when $\delta$ is large enough, i.e., when users are ``advertisement-averse'' enough. Otherwise, the hybrid model is never preferred. This observation partially explains the different strategies for YouTube and Facebook. As we introduced at the beginning of this section, YouTube launched its paid but ad-free version, YouTube Premium, as an alternative for its users, while Facebook has been hesitating to do so. Users are more ad-averse when they are streaming on YouTube than they are browsing their friends' posts on Facebook. If users on Facebook are not ad-averse enough, it will never be optimal for Facebook to choose the hybrid model and launch its subscription version with no ads.

In sum, Figure \ref{fig:mixed_choice_2} summarizes the platform's content moderation policy as well as its business model choice for different $\alpha$, $a$, and $\delta$ values. The shaded area is where the platform actively moderates content. 


\begin{figure}[h]
\caption{Optimal choice of business model and content moderation policy}\label{fig:mixed_choice_2}
\centering
\includegraphics[width=\textwidth]{figures/mixed_choice_2.PNG}
\end{figure}

All three plots in Figure \ref{fig:mixed_choice_2} have the same pattern for business model choice: the hybrid model can only be optimal when users' advertising value $a$ is intermediate, as well as users' ad aversion level $\delta$ is large, as stated in Proposition \ref{prop:hybrid_model_choice}). Also, for a small (large) $\alpha$, all business models induce an active (inactive) content moderation policy. For intermediate $\alpha$, when advertising and subscription models induce different moderation policies, we see that the hybrid model induces a similar moderation behavior as the advertising (subscription) model when $a$ is large (small), as stated in Proposition \ref{prop:hybrid_y}.

==> literatureReview.tex <==
\section{Related Literature} \label{sec: lit}

1. The first stream of research papers look at the users side, examining questions such as why and how users generate content. 

\cite{toubia2013intrinsic} compare intrinsic utility and image-related utility as two main reasons for people post UGC on Twitter. 

\cite{daugherty2008exploring} show that ego-defensive and social functional sources have the most explanatory power for creating UGC.

\cite{sun2017motivation} document an unexpected overall decrease in total UGC contribution after introducing monetary rewards and find a strong moderating effect of social connectedness.

\cite{iyer2016competing} theoretically analyze users' strategic decisions of whether to be a creator of UGC and then compete for the attention of receivers.


2. Past research also studies what information for a marketer to get from UGC and how to utilize it.

\cite{ghose2012designing} study how a platform can mine UGC to design a better ranking systems for its search engine.

\cite{timoshenko2019identifying} propose a machine learning-based approach for firms to identify customer needs for marketing strategy and product development from UGC.

\cite{iyengar2011opinion} study how content generated by opinion leaders and social contagion can affect new product adoption.

\cite{tirunillai2012does} examine the dynamics between UGC and stock performance.

\cite{goh2013social} compare the different impacts on consumer behavior of UGC and MGC: the effects vary by the type of directed or undirected communication modes by consumers and the marketer. 

3. Most research views UGC as an interchangeable concept as online WOM. A few papers consider UGC itself as a product that other users consume.

\cite{yildirim2013user} 

\cite{zhang2015differentiation}

\cite{albuquerque2012evaluating} evaluate the effectiveness of promotional activities in an online platform of UGC where users post content and purchase content by others.

\cite{ahn2016managing} builds a dynamic structural model of site participation, content generation, and content consumption to understand the evolution of UGC in
the context of a large number of heterogeneous users.

!! There is a new working paper on content moderation -- \cite{madio2020user}:
user base always goes down with content moderation


 - interaction with revenue models
 
 - AI technology use in content moderation



%{\bf [YI -- CAN YOU ADD SOME PAPERS ON CONTENT + SOCIAL MEDIA FROM MARKETING?]}


%Our paper contributes to the discussion on the ongoing policy debate about how online platforms should moderate content. Platforms, including Facebook and Twitter are pressured by policymakers to act in a timely manner to remove harmful content. Brands joined this wagon with a recent ``\#StopHateForProfit'' campaign, pulling their ads from social media platforms until Facebook and others do a better job in content moderation \citep{Morethan1000companies}.

This paper contributes to marketing literature in three ways. First, we contribute to the growing literature on social media and user generated content (UGC). 
A substantial body of research in marketing focused on social media and UGC, studying topics such as the reason why users contribute on social media \citep[e.g.,][]{toubia2013intrinsic,daugherty2008exploring}, the impacts of UGC \citep[e.g.,][]{iyengar2011opinion, tirunillai2012does, goh2013social}, the network effects of UGC on social media platforms \citep[e.g.,][]{zhang2015differentiation,susarla2012social}, new methods in analyzing UGC data \citep[e.g.,][]{ghose2012designing}, etc. 

1. look at user side: why and how users generate content

2. what information for a marketer to get from UGC and how to utilize it

3. theory papers on ugc
[positioning strategy: ]

-- how they model and how they are diff from ours -- wide range? 
 - Dina: the process of genearting WOM and manage WOM(?)
 - Differentiate product
 [In theoretical lit: do people (1) look at content management (promote some content) (2) prevent some content (product review removal? TripAdvisor - gets rid of most positive or most neg ones. fake reviews removal - empirical work)]
 
 fundamental diff: content moderation -- firm actively involved in pruning content: selecting people who can post. Other papers: self-selection by positioning. Exactly like target pricing -- ]
 



Based on our reading, this is the first theoretical paper on the strategy of content moderation for a self-interested social media platform. %While consumers directly experience a disutility  removal of the content 
Earlier literature has consistently demonstrated that individuals who have more extreme opinions relative to others are also more active in voicing them \citep{mathew2019spread} and enjoy a greater utility from doing so \citep{miller2009expressing,yildirim2013user}. We include this empirical fact in our modeling and allow users to vary in their enjoyment from posting and reading online content. 


Since most of content moderation is achieved through  algorithms, this paper also contributes to research on the economics of algorithms. As algorithms are increasingly more in charge of consumer screening in cases ranging from qualifying for a bank loan \citep{wei2015credit}, hiring \citep{cowgill2019economics, lee2018understanding}, online dating \citep{abeliuk2019price} to being served an ad \citep{lambrecht2019algorithmic},  they are also increasingly in use by platforms for UGC screening. This aspect of algorithms have not been studied in marketing. 


As this paper was being written, the Federal Law in the U.S. did not provide users options to challenge social media outlets' decisions to remove a content \citep{Brannon2019}. However, numerous other countries have taken legal actions to enforce social media companies to remove extreme content per regulations. Germany has passed a law in 2017, for instance, to enforce large\footnote{With greater than 2 million users.} social media platforms to accept and respond to user complaints about extreme content within 24 hours of receiving it \citep{Gesley2019}. %In more stringent enforcement examples, Malaysia passed a law in 2018 to punish any individual ``who maliciously creates, offers, publishes, prints, distributes, circulates or disseminates any fake news or publication containing fake news \citep{Buchanan2019}.'' 
As a remedy,  businesses now largely rely on artificial intelligence (AI) technologies to automatically detect and remove UGC believed to be harmful. Unfortunately, such detection technologies are less than perfect as the CEO of Facebook Mark Zuckerberg acknowledges,  ``removing hateful content from the site [is] difficult and beyond the capacity of artificial intelligence.'' \citep{EUthreatens}. We  contribute to the growing literature on algorithms by demonstrating that advertising vs. subscription revenue sources determine the incentives for investing into AI development, and the quality of technology is not independent of a firm's profit function, as Zuckerberg believes it to be.  


%Moreover, there is a concern about harming viewpoint diversity, where some groups' content and accounts are flagged more often than others. To mitigate the risk of disproportionately removing the content of some groups, online platforms integrate fairness concerns into content censoring algorithms. But it is not clear if integration of fairness, or yet alone monitoring and removing user-generated content is good for online platforms. 



\begin{comment}

\textcolor{blue}{
Recently there is a discussion for the possibility of subscription-based social media platforms. 
\url{https://www.businessinsider.com/subscription-platforms-patreon-substack-quality-alternative-to-social-media-2019-8}
\url{https://marketingland.com/can-ad-free-subscription-based-social-network-exist-189614}
\url{https://businessesgrow.com/2018/01/03/social-network-subscriptions/}
It is claimed in business reports that subscription-based may free users from toxic content on the platform. However, contrary to what is discussed in these business reports, a subscription-based platform may actually contain more extreme content... (Gab).
Actually we show that subscription model may make it more likely to be content moderation free.
}

\end{comment}

